Revisiting Selectional Preferences for Coreference Resolution

Selectional preferences have long been claimed to be essential for coreference resolution. However, they are mainly modeled only implicitly by current coreference resolvers. We propose a dependency-based embedding model of selectional preferences which allows fine-grained compatibility judgments with high coverage. We show that the incorporation of our model improves coreference resolution performance on the CoNLL dataset, matching the state-of-the-art results of a more complex system. However, it comes with a cost that makes it debatable how worthwhile such improvements are.

==> rel.tex <==
\section{Related Work}

Early work models selectional preferences with predicate argument frequencies, increased coverage through WordNet classes:

\cite{dagan90} word-word frequencies, eat chicken, low coverage

\cite{resnik93} word-class frequencies, eat FOOD, classes from WordNet, higher coverage through generalization

\cite{agirre01} class-class frequences, INGEST FOOD, even higher coverage

Similarity-based generalization:

\cite{erk07} learn selectional preferences on small annotated corpus, learn word similarities on large generalization corpus.

\cite{erk08} Structured Vector Space model, inverse selectional preferences

\cite{ritter10} LDA model

% TODO van den Cruys 2011? and 2014

All related work has small relation inventory, mostly subject - predicate, predicate - direct object

% TODO find and discuss work on selectional preferences over FrameNet


Prior work on integrating world knowledge into coreference resolution:

Frame-semantic \cite{erk07,rahman11b}

Semenatic roles \cite{ponzetto06b}

Word knowledge \cite{ponzetto06a}

\cite{durrett13b} Shallow semantics, very limited notion of selectional preferences via small number of latent word clusters derived from GigaWord, ``We use twenty clusters, which include clusters like president and leader (things which announce).'' Do not ablate semantic features, so it is not clear whether improvements comes from clusters or features like number and gender.

